Characterizing the Daytime Sextantids Meteor Shower and Unveiling the Nature of the Phaethon-Geminid Stream Complex

The Daytime Sextantids meteor shower, part of the Phaethon-Geminid Stream Complex (PGC), is closely related to the Geminids, currently the strongest meteor shower visible at the Earth. The DSX share a similar orbit to asteroid 2005 UD, but the nature of the association remains unclear. From optical data we find that DSX meteors ablate similarly to Geminids, suggesting that they are also high density and consistent with a common origin. From radar data we have isolated 19,007 DSX orbits through application of a novel convex hull approach to determine stream membership. We find at the peak the mean semi-major axis is near 1 AU, eccentricity is 0.86 and that both decrease as a function of solar longitude. The inclination averages 25 degrees at the peak but increases over time. Noticeable DSX activity extends from solar longitude 173-196$^{\circ}$ with a flux plateau between 186 - 189$^{\circ}$. The peak flux is $2 \pm 0.05 \times 10^{-3}$ km$^{-2}$ hr$^{-1}$, equivalent to a ZHR of 20. We estimate a true differential mass index for the shower of $s = 1.64 \pm 0.06$ at the time of peak and an average of $1.70 \pm 0.07$ for days surrounding the peak. The mass of the DSX stream is estimated to be $10^{16}$ g, the same order as 2005 UD, suggesting the stream is too massive to have been created by recent meteoroid production from 2005 UD. We propose that the DSX and 2005 UD were created in the same break-up event that created 3200 Phaethon.

==> DSX Source Code/project-intro-background-material.tex <==
Meteor showers are made up of individual meteors that share a common radiant. When viewed from the ground, a meteor’s radiant can be found from the path that it makes as it moves across the sky. For meteors that belong to the same meteor shower, these paths appear to converge on a single point in the sky, referred to as the meteor shower's radiant. For example, the radiant of the Daytime Sextantids meteor shower is located around its namesake, the Sextans constellation. Meteors that do not share the same radiant are called sporadic meteors and are not considered part of the shower. A focus of this study is to be able to define the radiant of the Daytime Sextantids meteor shower so that we can confidently separate the sporadic meteors from the DSX meteors.

==> project-intro-background-material.tex <==
Meteor showers are made up of individual meteors that share a common radiant. When viewed from the ground, a meteor’s radiant can be found from the path that it makes as it moves across the sky. For meteors that belong to the same meteor shower, these paths appear to converge on a single point in the sky, referred to as the meteor shower's radiant. For example, the radiant of the Daytime Sextantids meteor shower is located around its namesake, the Sextans constellation. Meteors that do not share the same radiant are called sporadic meteors and are not considered part of the shower. A focus of this study is to be able to define the radiant of the Daytime Sextantids meteor shower so that we can confidently separate the sporadic meteors from the DSX meteors.
